A Temporal Logic of Security

A new logic for verification of security policies is proposed. The logic, HyperLTL, extends linear-time temporal logic (LTL) with connectives for explicit and simultaneous quantification over multiple execution paths, thereby enabling HyperLTL to express information-flow security policies that LTL cannot. A model-checking algorithm for a fragment of HyperLTL is given, and the algorithm is implemented in a prototype model checker. The class of security policies expressible in HyperLTL is characterized by an arithmetic hierarchy of hyperproperties.

==> fig.purge.tex <==
\begin{figure}[t]
\setlength{\unitlength}{1mm}
	\centering
	\begin{picture}(50,25)%[width=6cm]
		\put(-12,9){$\purge(\pi)$}
	
		\put(10,10){\circle*{1}}
		\put(24,10){\circle*{1}}
		\put(38,10){\circle*{1}}
%		\put(40,10){\circle*{1}}
		\put(49,10){\dots}

		\put(11,10){\line(1,0){12}}
		\put(25,10){\line(1,0){12}}
		\put(39,10){\line(1,0){5}}

		\put(5,13){$(\lambda,l)$}
		\put(19,13){$(\lambda,l)$}
		\put(33,13){$(\lambda,l')$}
%		\put(39,13){$(\lambda,l_2)$}

		\put(-1,24){$\pi$}

		\put(10,25){\circle*{1}}
		\put(24,25){\circle*{1}}
		\put(38,25){\circle*{1}}
%		\put(40,25){\circle*{1}}
		\put(49,25){\dots}

		\put(11,25){\line(1,0){12}}
		\put(25,25){\line(1,0){12}}
		\put(39,25){\line(1,0){5}}

		\put(5,28){$(h',l)$}
		\put(19,28){$(h'',l)$}
		\put(33,28){$(h''',l')$}
%		\put(39,28){$(l_2,h_3)$}

	\end{picture}
	\caption{Paths $\pi$ and $\purge(\pi)$ have the same low inputs and outputs, but $\purge(\pi)$ has empty high inputs and outputs.\label{fig:noninterference}}
\end{figure}
